Dynamics of poroelastocapillary rise

A wetting liquid is driven through a thin gap due to surface tension and when the gap boundaries are elastic, the liquid deforms the gap as it rises. But when the fluid boundaries are also permeable (or poroelastic), the liquid can permeate the boundaries as the fluid rises and change their properties, for example by swelling and softening, thereby altering the dynamics of the rise. In this paper, we study the dynamics of capillary rise between two poroelastic sheets to understand the effects of boundary permeability and softening. We find that if the bending rigidity of sheets is reduced, due to liquid permeation, the sheets coalesce faster compared to the case of impermeable sheets. We show that as a direct consequence of this faster coalescence, the volume of fluid captured between the sheets can be significantly lower.

==> definitions.tex <==
\def\boldsymbol{\bm}

\def\para{\parallel}

\def \t{\tensorsym}
\def \lb{\left}
\def \rb{\right}
\def \ei{\eta_1}
\def \eii{\eta_2}

\def \d{\,\text{d}}
\def \n{\text{n}}

\def \absx{\left|\bx\right|}
\def \an{\lb|n\rb|}
\newcommand{\upc}[1]{\overset{\triangledown}{#1}}


\def \eps{\epsilon}
\def \veps{\varepsilon}

\def \etah{\hat{\eta}}
\def \bgamma{\boldsymbol{\gamma}}
\def \bgammadb{\bar{\dot{\boldsymbol{\gamma}}}}
\def \bgammadt{\tilde{\dot{\boldsymbol{\gamma}}}}
\def \bgammad{\dot{\boldsymbol{\gamma}}}
\def \bgammadh{\hat{{\dot{\bgamma}}}}
\def \gammad{{\dot{\gamma}}}
\def \muh{\hat{\mu}}
\def \bnabla{\boldsymbol{\nabla}}
\def \bnablap{\boldsymbol{\nabla}^\perp}
\def \omegah{\hat{\omega}}
\def \psib{\bar{\psi}}
\def \psit{\tilde{\psi}}
\def \psid{\dot{\psi}}
\def \bsigma{\boldsymbol{\sigma}}
\def \sigmah{\hat{\sigma}}
\def \bsigmah{\hat{\boldsymbol{\sigma}}}
\def \bsigmat{\tilde{\bsigma}}
\def \btau{\boldsymbol{\tau}}
\def \btaub{\bar{\boldsymbol{\tau}}}
\def \btaud{\dot{\boldsymbol{\tau}}}
\def \btaut{\tilde{\boldsymbol{\tau}}}
\def \btauh{\hat{\boldsymbol{\tau}}}
\def \brho{\boldsymbol{\rho}}
\def \bmu{\boldsymbol{\mu}}
\def \bdelta{\boldsymbol{\delta}}
\def \bDelta{\boldsymbol{\Delta}}
\def \bDeltah{\hat{\boldsymbol{\Delta}}}
\def \Deltab{\bar{\Delta}}
\def \Deltah{\hat{\Delta}}
\def \buprime{\boldsymbol{u^{\prime}}}

\def \vphi{\varphi}

\def \taud{\dot{\tau}}
\def \tauh{\hat{\tau}}
\def \thetad{\dot{\theta}}
\def \bxi{\boldsymbol{\xi}}

\def \bGamma{\mathbf{\Gamma}}
\def \bLambda{\mathbf{\Lambda}}
\def \bomega{\mathbf{\omega}}
\def \bomegat{\tilde{\mathbf{\omega}}}
\def \bOmega{\mathbf{\Omega}}
\def \bOmegah{\hat{\mathbf{\Omega}}}
\def \bOmegat{\tilde{\mathbf{\Omega}}}
\def \Psib{\bar{\Psi}}
\def \Psit{\tilde{\Psi}}
\def \bTheta{\mathbf{\Theta}}
\def \bPi{\mathbf{\Pi}}


\def \DeI{\text{D}_{\text{I}}}
\def \DeR{\text{D}_{\text{R}}}
\def \Deone{\De_1}
\def \Detwo{\De_2}
\def \T{\text{T}}
\def \Ar{\text{Ar}}
\def \Bi{\text{Bi}}
\def \Bo{\text{Bo}}
\def \Ca{\text{Ca}}
\def \Cu{\text{Cu}}
\def \Da{\text{Da}}
\def \De{\text{De}}
\def \La{\text{La}}
\def \M{\text{M}}
\def \Ma{\text{Ma}}
\def \Pe{\text{Pe}}
\def \Re{\text{Re}}
\def \Sc{\text{Sc}}
\def \St{\text{St}}
\def \SR{\dot{\text{S}}_{\text{R}}}
\def \Tr{\text{Tr}}
\def \UD{U_\Delta}
\def \UDone{U_{\Delta 1}}
\def \UDtwo{U_{\Delta 2}}
\def \UDthree{U_{\Delta 3}}
\def \UDfour{U_{\Delta 4}}
\def \UDm{U_{\Delta m}}


\def \bA{\mathbf{A}}
\def \bAt{\tilde{\mathbf{A}}}
\def \bB{\mathbf{B}}
\def \bBt{\tilde{\mathbf{B}}}
\def \bC{\mathbf{C}}
\def \bD{\mathbf{D}}
\def \bE{\mathbf{E}}
\def \bF{\mathbf{F}}
\def \bFt{\tilde{\mathbf{F}}}
\def \bG{\mathbf{G}}
\def \bH{\mathbf{H}}
\def \bHt{\tilde{\mathbf{H}}}
\def \bI{\mathbf{I}}
\def \bJ{\mathbf{J}}
\def \bK{\mathbf{K}}
\def \bL{\mathbf{L}}
\def \bM{\mathbf{M}}
\def \bN{\mathbf{N}}
\def \bP{\mathbf{P}}
\def \bR{\mathbf{R}}
\def \bS{\mathbf{S}}
\def \bT{\mathbf{T}}
\def \bU{\mathbf{U}}
\def \bUt{\tilde{\mathbf{U}}}
\def \bV{\mathbf{V}}
\def \bW{\mathbf{W}}
\def \bX{\mathbf{X}}

\def \Rh{\hat{R}}
\def \Uh{\hat{U}}


\def \bEh{\hat{\mathbf{E}}}
\def \bFh{\hat{\mathbf{F}}}
\def \bKb{\bar{\mathbf{K}}}
\def \bLh{\hat{\mathbf{L}}}
\def \bRh{\hat{\mathbf{R}}}
\def \bUh{\hat{\mathbf{U}}}
\def \bXh{\hat{\mathbf{X}}}

\def \Fh{\hat{F}}

\def \ba{\mathbf{a}}
\def \bah{\hat{\mathbf{a}}}
\def \bb{\mathbf{b}}
\def \bbh{\hat{\mathbf{b}}}
\def \bc{\mathbf{c}}
\def \bdh{\hat{\mathbf{d}}}
\def \bd{\mathbf{d}}
\def \be{\mathbf{e}}
\def \beh{\hat{\mathbf{e}}}
\def \bet{\tilde{\mathbf{e}}}
\def \bf{\mathbf{f}}
\def \bft{\tilde{\mathbf{f}}}
\def \bg{\mathbf{g}}
\def \bi{\mathbf{i}}
\def \bih{\hat{\mathbf{i}}}
\def \bj{\mathbf{j}}
\def \bjh{\hat{\mathbf{j}}}
\def \bk{\mathbf{k}}
\def \bkh{\hat{\mathbf{k}}}
\def \bl{\mathbf{l}}
\def \blh{\hat{\mathbf{l}}}
\def \bn{\mathbf{n}}
\def \bp{\mathbf{p}}
\def \br{\mathbf{r}}
\def \bs{\mathbf{s}}
\def \bt{\mathbf{t}}
\def \bu{\mathbf{u}}
\def \uh{\hat{u}}
\def \but{\tilde{\mathbf{u}}}
\def \bv{\mathbf{v}}
\def \bx{\mathbf{x}}
\def \bxt{\tilde{\mathbf{x}}}
\def \bz{\mathbf{z}}

\def \at{\tilde{a}}
\def \ct{\tilde{c}}
\def \dt{\tilde{d}}
\def \ft{\tilde{f}}
\def \gt{\tilde{g}}
\def \pt{\tilde{p}}
\def \qt{\tilde{q}}
\def \ut{\tilde{u}}
\def \vt{\tilde{v}}

\def \ed{\dot{e}}
\def \fd{\dot{f}}
\def \md{\dot{m}}
\def \xd{\dot{x}}
\def \rd{\dot{r}}
\def \Qd{\dot{Q}}
\def \Rd{\dot{R}}
\def \yd{\dot{y}}
\def \zd{\dot{z}}
\def \Zd{\dot{Z}}
\def \gd{\dot{g}}
\def \Pd{\dot{P}}
\def \Gd{\dot{G}}
\def \Fd{\dot{F}}
\def \xdd{\ddot{x}}
\def \rdd{\ddot{r}}
\def \ydd{\ddot{y}}
\def \zdd{\ddot{z}}
\def \etad{\dot{\eta}}
\def \xid{\dot{\xi}}
\def \rdd{\ddot{r}}
\def \ydd{\ddot{y}}
\def \zdd{\ddot{z}}
\def \phid{\dot{\phi}}
\def \thetad{\dot{\theta}}

\def \hb{\bar{h}}
\def \ph{\hat{p}}
\def \yh{\hat{y}}

\def \Eb{\bar{E}}
\def \Et{\tilde{E}}
\def \Gammat{\tilde{\Gamma}}
\def \Pit{\tilde{\Pi}}
\def \bnablat{\tilde{\boldsymbol{\nabla}}}
\def \nablat{\tilde{\nabla}}

\def \yt{\tilde{y}}
\def \bzero{\mathbf{0}}

\def \kappab{\bar{\kappa}}

\def \bfh{\hat{\bf}}
\def \bnh{\hat{\bn}}
\def \bth{\hat{\bt}}
\def \brd{\dot{\br}}
\def \brt{\tilde{\br}}
\def \brh{\hat{\br}}
\def \buh{\hat{\bu}}
\def \but{\tilde{\bu}}
\def \buinf{\bu_\infty}
\def \bxd{\dot{\bx}}
\def \bxh{\hat{\bx}}
\def \byd{\dot{\by}}

\def \Af{\mathcal{A}}
\def \Bf{\mathcal{B}}
\def \Cf{\mathcal{C}}
\def \Ef{\mathcal{E}}
\def \Ff{\mathcal{F}}
\def \Ffh{\hat{\mathcal{F}}}
\def \Gf{\mathcal{G}}
\def \Hf{\mathcal{H}}
\def \Kf{\mathcal{K}}
\def \Lf{\mathcal{L}}
\def \Lfh{\hat{\mathcal{L}}}
\def \Mf{\mathcal{M}}
\def \Nf{\mathcal{N}}
\def \Of{\mathcal{O}}
\def \Pf{\mathcal{P}}
\def \Rf{\mathcal{R}}
\def \Rfh{\hat{\mathcal{R}}}
\def \Uf{\mathcal{U}}
\def \Ufh{\hat{\mathcal{U}}}

\def \ta{\mathsf{\t a}}
\def \tb{\mathsf{\t b}}

\def \tzero{\mathsf{\t 0}}

\def \tA{\mathsf{\t A}}
\def \tE{\mathsf{\t E}}
\def \tF{\mathsf{\t F}}
\def \tG{\mathsf{\t G}}
\def \tH{\mathsf{\t H}}
\def \tK{\mathsf{\t K}}
\def \tL{\mathsf{\t L}}
\def \tR{\mathsf{\t R}}
\def \tS{\mathsf{\t S}}
\def \tT{\mathsf{\t T}}
\def \tU{\mathsf{\t U}}



\def \tAh{\mathsf{\t{\hat{A}}}}
\def \tEh{\mathsf{\t{\hat{E}}}}
\def \tFh{\mathsf{\t{\hat{F}}}}
\def \tGh{\mathsf{\t{\hat{G}}}}
\def \tHh{\mathsf{\t{\hat{H}}}}
\def \tKh{\mathsf{\t{\hat{K}}}}
\def \tLh{\mathsf{\t{\hat{L}}}}
\def \tRh{\mathsf{\t{\hat{R}}}}
\def \tSh{\mathsf{\t{\hat{S}}}}
\def \tTh{\mathsf{\t{\hat{T}}}}
\def \tUh{\mathsf{\t{\hat{U}}}}

\def \Ts{T^*}
\def \Tsd{\dot{T}^*}
\def \Tsdd{\dot{T}^{2*}}

\def \eq{\text{eq}}
\def \on{\text{on}}
\def \ss{\text{ss}}
\def \off{\text{off}}
\def \max{\text{max}}
